App Review Driven Collaborative Bug Finding

Software development teams generally welcome any effort to expose bugs in their code base. In this work, we build on the hypothesis that mobile apps from the same category (e.g., two web browser apps) may be affected by similar bugs in their evolution process. It is therefore possible to transfer the experience of one historical app to quickly find bugs in its new counterparts. This has been referred to as collaborative bug finding in the literature. Our novelty is that we guide the bug finding process by considering that existing bugs have been hinted within app reviews. Concretely, we design the BugRMSys approach to recommend bug reports for a target app by matching historical bug reports from apps in the same category with user app reviews of the target app. We experimentally show that this approach enables us to quickly expose and report dozens of bugs for targeted apps such as Brave (web browser app). BugRMSys's implementation relies on DistilBERT to produce natural language text embeddings. Our pipeline considers similarities between bug reports and app reviews to identify relevant bugs. We then focus on the app review as well as potential reproduction steps in the historical bug report (from a same-category app) to reproduce the bugs. Overall, after applying BugRMSys to six popular apps, we were able to identify, reproduce and report 20 new bugs: among these, 9 reports have been already triaged, 6 were confirmed, and 4 have been fixed by official development teams, respectively.

==> Background.tex <==
\section{Background}\label{sec:background}

==> bios.tex <==


\begin{wrapfigure}{l}{0.2\textwidth}
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/tang.jpeg}%
\end{wrapfigure}\par
\textbf{Xunzhu Tang} is PhD student with the Interdisciplinary Centre for Security, Reliability and Trust (SnT) at the University of Luxembourg. He received his master degree in Computer System and Architecture from Huazhong University of Science and Technology, China in 2021. His research interests include patch explanation, bug finding and fixing.
\newline
\par
\mbox{} \\

\begin{wrapfigure}{l}{0.2\textwidth}
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/haoye.png}%
\end{wrapfigure}\par
\textbf{Haoye Tian} is PhD student with the Interdisciplinary Centre for Security, Reliability and Trust (SnT) at the University of Luxembourg. He received his master degree in Software Engineering from Chongqing University, China in 2019. His research interests include automated program repair, patch validation, machine and deep learning.
\newline
\par
\mbox{} \\

\begin{wrapfigure}{l}{0.2\textwidth}
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/kuiliu.jpg}%
\end{wrapfigure}\par
\textbf{Kui Liu} is an associate professor in Software Engineering at the College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics, China. He received the MS degree in computer application technology at Southwest University (Chongqing, China) in 2013, and obtained the Ph.D. degree in computer science at the University of Luxembourg in 2019. His research interests include automated program repair, automated fault localization, fix pattern mining, deep learning, and empirical software engineering.
\newline
\par
\mbox{} \\

\begin{wrapfigure}{l}{0.2\textwidth}
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/Xinxia.jpeg}%
\end{wrapfigure}\par
\textbf{Xin Xia} is the director of the Software Engineering Application Technology Lab at Huawei, China. He received the ACM SIGSOFT Early Career Researcher Award in 2022. His current research focuses on data science for software engineering, i.e., mining and analyzing rich data in software repositories to uncover interesting and actionable information
\par
\mbox{} \\

\begin{wrapfigure}{l}{0.2\textwidth}
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/jacques-03.png}%
\end{wrapfigure}\par
\par
\textbf{Jacques Klein} is a researcher and professor in software engineering and software security who develops innovative approaches and tools towards helping the research and practice communities build trustworthy software. He is a member of the Interdisciplinary Centre for Security, Reliability and Trust (SnT) at the University of Luxembourg. He received a Ph.D. degree in Computer Science from the University of Rennes, France, in 2006. His main areas of expertise are threefold: (1) Software Security (Malware detection, prevention and dissection, Static Analysis for Security, Vulnerability Detection, etc.); (2) Software Reliability (Software Testing, Semi-Automated and Fully-Automated Program Repair, etc.); (3) Data Analytics (Multi-objective reasoning and optimization, Model-driven data analytic, Time Series Pattern Recognition, etc.).
\par
\mbox{} \\


\begin{wrapfigure}{l}{0.2\textwidth}
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/biss.png}%
\end{wrapfigure}\par
\textbf{Tegawend{\'e} F. Bissyand{\'e}} 
is research scientist with the Interdisciplinary Center for Security, Reliability and Trust at the University of Luxembourg. He holds a PhD in computer from the Universit{\'e} de Bordeaux in 2013, and an engineering degree (MSc) from ENSEIRB. His research interests are in debugging, including bug localization and program repair, as well as code search, including code clone detection and code classification. He has published research results in all major venues in Software engineering (ICSE, ESEC/FSE, ASE, ISSTA, EMSE, TSE). His research is supported by FNR (Luxembourg National Research Fund). Dr. Bissyand{\'e} is the PI of the CORE RECOMMEND project on program repair, under which the current work has been performed.
\par
\mbox{} \\



==> tool_generality.tex <==
\section{Tool}\label{sec:generality}

\subsection{Tool of Crawling Github Data}
\subsection{Tool of Crawling App Reviews}
\subsection{Easy-to-use API}
